White Paper on Radio Channel Modeling and Prediction to Support Future Environment-aware Wireless Communication Systems

COST INTERACT working group (WG)1 aims at increasing the theoretical and experimental understanding of radio propagation and channels in environments of interest and at deriving models for design, simulation, planning and operation of future wireless systems. Wide frequency ranges from sub-GHz to terahertz (THz), potentially high mobility, diverse and highly cluttered environments, dense networks, massive antenna systems, and the use of intelligent surfaces, are some of the challenges for radio channel measurements and modeling for next generation systems. As indicated in [1], with increased number of use cases (e.g., those identified by one6G [2] and shown in Fig. 1) to be supported and a larger number of frequency bands, a paradigm shift in channel measurements and modeling will be required. To address the particular challenges that come with such a paradigm shift, WG1 started the work on relevant topics, ranging from channel sounder design, metrology and measurement methodologies, measurements, modeling, and systematic dataset collection and analysis. In addition to the core activities of WG1, based on the strong interest of the participants, two sub-working groups (subWGs) have been initiated as part of WG1: i) subWG1.1 on millimeter-wave (mmWave) and THz sounding (subWG THz) and ii) subWG1.2 on propagation aspects related to reconfigurable intelligent surfaces (RIS) (subWG RIS). This white paper has two main goals: i) it summarizes the state-of-theart in radio channel measurement and modeling and the key challenges that the scientific community will have to face over the next years to support the development of 6G networks, as identified by WG1 and its subWGs; and ii) it charts the main directions for the work of WG1 and subWGs for the remainder of COST INTERACT duration (i.e., until October 2025).

==> 6.1Xuesong.tex <==
\iffalse
\textcolor{red}{Please include some references to relate to COST INTERACT work\\}
\textcolor{blue}{Xuesong: Going through all previous TDs, I was able to find 5 related TDs (22)02042, (22)02046, (23)04049, (23)05029 and (23)05036. The first two proposed new estimation algorithms based on maximum likelihood and machine learning (auto-encoder), respectively. The last three applied HRPE algorithms for their channel measurements (didn't propose new algorithms). Should I only include the first two or all of them? And for reference, should I replace the TD number with its corresponding published version (if any)? Many thanks! (I will continue after vacation on Wednesday, Jun 7.) }
\textcolor{red}{Mate: Please include a reference to the publicly available versions (conference/journal) of the first two TDs; up to you regarding the remaining ones. Check out the footnote in intro: ``While COST INTERACT contributions are not made public, vast majority of contributions are published in conferences, journals, or other venues, either before or after submission to COST INTERACT. Throughout the paper, we refer to those publicly available versions of contributions.''} 
\textcolor{blue}{Xuesong: Turns out that the first TD (22)02042 is not published, neither in conference, journal nor arxiv. So I only discussed the second TD as below. } 
\textcolor{red}{Wei: the comment part above can be deleted now.}
\fi
\textcolor{black}{Channel parameter estimation aims at extracting propagation parameters such as propagation delay, angles, polarimetric amplitudes, etc. of path components from the measurement data. COST INTERACT has contributed to the development of such algorithms. For example, the authors in \cite{9909796} proposed a maximum-likelihood estimation algorithm to deal with channels that exhibit a mixture of independent \glspl{dmc}, which is in contrast to the commonly assumed model of single \gls{dmc} mode. An auto-encoder was proposed to infer the order of \gls{dmc} modes and for initializing the parameters of the \gls{dmc}s.} In general, channel parameter estimation techniques can be mainly classified into four categories: spectra-based techniques, subspace-based techniques, sparsity-recovery-based techniques, and maximum-likelihood-based techniques.
\subsubsection{Spectra-based techniques}

%\cite{526899}

Bartlett beamforming is the most classical spectra-based method, \textcolor{red}{aiming to find the direction(s) with dominant power(s) \cite{526899}}. Its variant, a frequency-invariant beamformer for uniform circular arrays can also be found in \cite{7523340}. \textcolor{red}{The basic idea was to pre-compensate to frequency-dependent phase variation so that \gls{2d}-\gls{fft}, i.e., beamforming,} can be efficiently applied to finding the dominant paths in azimuth and delay domains jointly. For \gls{mmwave} frequency bands, a widely applied spectra-based method is to obtain the joint angle-delay spectrum according to the channel measurements by rotating horn antennas to different directions \cite{8103059,8094309,7400962,7109864}. These methods are straightforward and with relatively lower complexity. However, system responses such as antenna radiation patterns are usually embedded in the resulting spectra, making it difficult to separate the propagation channels from the sounder hardware, not to mention the low resolutions. 
\subsubsection{Subspace-based techniques}
Among the subspace-based methods, the well-known ones are \gls{music} \textcolor{red}{\cite{1143830}} and \gls{esprit} \textcolor{red}{\cite{1457851}}, and their variants can be found in, e.g., \cite{8093607,1395953,575559,8316940,552142}. In the early development of these techniques, the basic assumption is that propagation paths are uncorrelated so that the covariance matrix of the received signals can be decomposed into signal subspace and noise subspace \textcolor{red}{\cite{1143830}. By examing the distances (orthogonality) between steering vectors and the noise space, a spectrum can be obtained with its peaks indicating path directions. Intuitively, if a steering vector is orthogonal to the noise space, it means that it belongs to the signal space, i.e., contributing to the  received signals.} Later on, these techniques were extended to dual domains such as delay vs. frequency covariance matrix. The main limitation is the deficiency in resolving a large number of paths and requiring a certain number of snapshots to obtain a sample covariance matrix. 
\subsubsection{Sparsity-recovery-based techniques}
Sparsity recovery algorithms \cite{7390019,8122055} are developed based on the assumption that the channel exhibits sparsity in parameter domains, \textcolor{red}{i.e., only a few paths contributing to the received signals}, although the assumption is still questionable even in \gls{mmwave} frequency bands \cite{8386686}. By exploiting specific optimization principles, e.g., convex optimization, channel parameters can be recovered. 
\subsubsection{Maximum-likelihood-based techniques}
Despite the high complexity of maximum-likelihood-based estimation algorithms, they can extract the propagation parameters that are properly defined in the signal model with a high resolution that approaches the theoretic lower error bound, i.e., \gls{crlb}. The most widely used maximum-likelihood-based algorithm is the \gls{sage} algorithm \cite{753729}. It is a further enhanced algorithm based on the \gls{em} principle \cite{543975} that is theoretically proven to converge to a local maximum of the likelihood objective function. In \gls{sage}, the high-dimensional estimation/optimization problem can be decomposed into several one-dimensional problems, leading to much lower complexity and faster convergence. In \cite{8713575,9104014,9115069}, variants of the \gls{sage} algorithm can also be found for \gls{mmwave} wideband large-scale arrays, where the trajectories in delay domain across the array aperture are exploited for effective initializations and interference cancellation. The \gls{sage} algorithm usually assumes that the propagation paths are well-resolvable. However, it is possible that due to the scattering effect of rough surfaces, the resulting \gls{mpc}s can be very dense in delay and angle domains that cannot be well resolved by the intrinsic ability of the sounder. In such cases, one needs to modify the signal model to consider these dense \gls{mpc}s, i.e., \glspl{dmc}, as colored noises (in addition to white Gaussian noises) with certain power profiles for a better estimation of other discrete \gls{mpc}s, which is basically the RIMAX algorithm \cite{RICHTER1}. Although there exist not a few different parameter estimation techniques, future \gls{mmwave} and \gls{thz} propagation channels will pose more challenges due to much larger bandwidths, much larger array apertures, etc. Spherical-wave propagation, channel birth-death on the array, frequency-dependent responses of antennas and sounders, etc., will make the signal model much more complicated, meaning that low-complexity yet still high-resolution estimation techniques are still in need.

Another important consideration for parameter estimation is that the system response of the channel sounder must be well characterized for a realistic signal model. Otherwise, the mismatch of the signal model from reality can result in many ghost (erroneous) paths estimated \cite{THzMagazine}. The response of cables, power amplifiers, filters, converters, etc., of the channel sounder can be easily calibrated through back-to-back measurements, i.e., directly connecting Tx and Rx without antennas. For antennas or antenna arrays, they can be placed in an anechoic chamber to measure the \gls{3d} responses of antenna elements at discrete angles. The measurement data can be later on exploited to interpolate the responses at arbitrary angles. There are different ways to do this, which include direct (linear or non-linear) interpolation, spherical harmonics, and \gls{eadf} \cite{EADF}. Direct interpolation is straightforward but non-analytic. Alternatively, one can transform the measured pattern from the spatial domain to another domain using basis functions, either spherical harmonics or Fourier basis (\gls{eadf}). Using a forward transform, the transformed spectra are obtained and then utilized to recover spatial patterns. There is also a possibility to compress the measurement data if the spectra are concentrated so that the unimportant components in the transformed domain can be removed. A practical application of \gls{eadf} in dynamic \gls{mmwave} channel sounding using 128$\times$256 switched arrays can be found in \cite{mmWavesounder}.

%\subsubsection{Future work\textcolor{red}{? Please rephrase or modify title if not appropriate} \textcolor{blue}{Xuesong: Better use Future challenges and directions?} }
\subsubsection{Future challenges and directions}
6G is envisioned to support applications beyond the current
5G mobile use scenarios, which will pose stringent
requirement on the communication systems in terms of data-rate, latency, reliability, and so on. To meet those demanding requirements, a raft of advanced radio technologies are envisioned, e.g.  utilization of  higher
frequency spectra (e.g. up to sub-\gls{thz} frequency bands), higher system bandwidth (e.g. up to a few GHz), and larger-scale
multi-antenna systems (e.g. large-scale or extremely large-scale antenna), utilization of \gls{ris}, etc. The advancement in 6G radio technologies have posed significant challenges to the channel estimation parameter. For example, the extremely large scale antenna array will bring a few new challenges for the channel parameter estimation: near-field and spatial non-stationary effects. State-of-the-art algorithms, which are developed based on plane
wave model and spatial stationary channel might fail to address all the new features introduced by the massive \gls{mimo} systems. The narrow-band assumption might also be violated for 6G radio systems that potentially utilize the ultra-wide-band technology, which should be properly considered for developing channel parameter estimator. As for the sub-\gls{thz}/\gls{mmwave} channel measurements, the required phase accuracy might be difficult to achieve, though a few works on phase compensation concept have been reported to achieve coherent phase measurement for virtual antenna array systems. Therefore, it would be desirable to develop channel parameter estimators, which is robust to phase measurement inaccuracy. 

